Vehicular Inter-Networking via Named Data

In this paper we apply the Named Data Networking, a newly proposed Internet architecture, to networking vehicles on the run. Our initial design, dubbed V-NDN, illustrates NDN's promising potential in providing a unifying architecture that enables networking among all computing devices independent from whether they are connected through wired infrastructure, ad hoc, or intermittent DTN. This paper describes the prototype implementation of V-NDN and its preliminary performance assessment.

==> demonstration_copy.tex <==
\section{Demonstration Setup}
\label{sec:demonstration}
\name has been implemented as proof of concept prototype at UCLA and tested in campus  using  UCLA  Vehicular Testbed. Several experiments were performed on November 25, November 30, and December 1st, 2012, the first day was a clear day while the other two were raining days. The experiments involved multiple vehicles. In particular we used 6 vehicles on Nov 25, 2012, 10 vehicles on November 30th 2012, and 9 vehicles on December 1st 2012.  We designed and implemented two NDN applications for the vehicular domain; the {\bf Info-Traffic} application and the {\bf Road-Photo Application}. The info-traffic application emulates the request of traffic information for a specific area and the response from a vehicle that has recently been in such area likewise the road-photo application emulates the request of a picture for a specific area and the response from a vehicle that has recently been in that area.  The  area is encoded in the name and rather than coordinates we refer to intersections and streets stemming from that intersections \ie /traffic/westwood-at-strathmore/ would refer to the traffic information from the area close to the Westwood-Strathmore intersection in the UCLA campus.  A car that has been or is currently in such location will respond to the interest reporting the proper traffic information. Is worth noticing that multiple responses may be generated by one interest  however, in the current implementation,  only the first response is considered.  We employed two different types of mobility pattern: \emph{Urban Platooning} with the cars going around a large urban block or a parking lot in a single line platoon, and a more realistic mobility which we call \emph{double-clock} where a part of the available vehicles run in clockwise loops around a block and another disjoint set of cars runs in a counter-clockwise block in an adjacent block thus vehicles from different loops can communicate roughly only half of the time; figure \ref{fig:clockwiseroute} and \ref{fig:counterclockwiseroute} show the route details for the two groups of vehicles.  

The experiments were designed to investigate \name behavior in  the following communication scenarios typical for the vehicular applications domain.
\begin{itemize}

\item {\bf V2V}: Interests and content travel through WiFi Vehicle-to-Vehicle Connections thus the content addressed is relatively local (\ie few hops away). Applications such as assisted left-turns and accident warnings may benefit from this type of communications (figure \ref{fig:V2VRoute})

\item {\bf I2V}: Lets consider a traffic monitoring system that constantly requests the current status for various critical intersections. The consumer node resides on the wired network (\ie traffic control center) and the producer node resides on the vehicular network \ie vehicles that are close or have been recently close to a point of interest (figure\ref{fig:I2VRoute}).

\item {\bf V2I}: The producer is connected to the wired network while the consumer is on the vehicle.  A typical example is when a vehicle wants to retrieve data about the traffic in the destination and direct v2v routing may be inefficient or even not possible (figure\ref{fig:V2IRoute}).
 
\item {\bf resilience to disruption}: Vehicular networks are prone to disruption, the link duration is relatively short and the topology is continuosly changing resulting in dynamic network partitions \cite{rowstron2009characteristics}. We designed a set of experiments to reproduce this phenomena and study NDN behavior/performance  in such harsh conditions. 

\item {\bf in-network storage}: One of the great innovations of the Named Data Network  paradigm is to introduce caching in the network.  This feature improves efficiency and  turns out to be  essential for VANETs.  
\end{itemize}

\begin{figure*}[htdp]
\begin{minipage}[htdp]{\textwidth}
\centering{
\subfigure[\name Driving Route, Clock Wise  one block around Parking Lot 8]{
\includegraphics[width=0.30\textwidth]{figures/Driving-Clockwise}
\label{fig:clockwiseroute}
}
\hfil
\subfigure[\name Driving Route, Clock Wise two blocks around Parking Lot 8]{
\includegraphics[width=0.30\textwidth]{figures/Driving-CounterClockwise}
\label{fig:counterclockwiseroute}
}
\hfil
\subfigure[\name V2X experiment: Mobility pattern and AP placement]{
\includegraphics[width=0.23\textwidth]{figures/Lot32-MultiHoming.png}
\label{fig:car2XLot32}
} 
}
\caption{Mobility Patterns}
\label{fig:MobilityPatterns}
\end{minipage}
\end{figure*}
\subsection{Field Experiments}
We performed a number of field experiments for both applications varying the mobility patterns and the type of communication involved (\ie V2V, V2I/I2V, V2V2I). Each experiment was repeated several times. The experiments are summarized in table \ref{tab:experiments}
\begin{table}[htdp]
\caption{Experiment Summary}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Exp. \#&Application&Type & Mobility\\
\hline
A.1&Info-Traffic&V2V&P8:Still \& \\
&&&Urban Platoon\\
\hline
A.1&Info-Traffic&V2V&P8:Still \& \\
&&&Urban Platoon\\
\hline
A.3&Info-Traffic&V2V&Fig.~\ref{fig:clockwiseroute}~\&~\ref{fig:counterclockwiseroute}\\
\hline
A.4&Road-Photo&V2V&Fig.~\ref{fig:clockwiseroute}~\&~\ref{fig:counterclockwiseroute}\\
\hline
\hline
B.1&Info-Traffic&V2V&P8:Still \& \\
&&&Urban Platoon\\
\hline
B.2&Info-Traffic&V2V&P8:Still \& \\
&&&Urban Platoon\\
\hline
B.3&Info-Traffic&V2V2I&Fig.~\ref{fig:clockwiseroute}~\&~\ref{fig:counterclockwiseroute}\\
\hline
B.4&Road-Photo&V2V2I&Fig.~\ref{fig:clockwiseroute}~\&~\ref{fig:counterclockwiseroute}\\
\hline
\end{tabular}
\end{center}
\label{tab:experiments}
\end{table}%
\subsubsection{{\bf Experiments A1, A2, B1, B2}}  are preliminary experiments performed on the rooftop of UCLA parking structure  P8 with with \emph{no mobility} or very basic \emph{slow urban platooning}. UCLA P8 rooftop is 265m long and 76m large. The wireless range was  to cover the whole roof at the operating frequency of 2.4GHz; however due to a very large number of competing transmitters (net-stumbler reports about 100 access points that can be eared in that area) the radio range using broadcast messages unexpectedly ranged from 1m to 30m. Additional experiments performed in ideal conditions at the \emph{El Mirage Dry Lake Bed} ( 34\degree 37'50.10"N, 117\degree 34'14.64"W), in California show that with no-interference an 2.4GHz wifi interface can achieve up to 550m.

\subsubsection{{\bf Experiments A3, A4, B3, B4}} were performed on the roads around UCLA structure P8. The pool of 10 vehicles has been divided in two groups of 6 and 4 cars respectively. The smallest group of vehicle was running clockwise on around the P8 Block as shown in fig. \ref{fig:clockwiseroute}. The second (and largest) part of vehicles was running counterclockwise to cover a larger road block which also includes the UCLA P8 structure see figure \ref{fig:counterclockwiseroute}. Car speeds ranged from 6.3$_{m/s}$ to 21.2$_{m/s}$  \ie {\raise.17ex\hbox{$\scriptstyle\sim$}}14 to 47mph. The mobility pattern allows vehicles traveling in opposite direction to meet however prevents a continuos connectivity between the two partitions. In particular, the small loop shown in figure \ref{fig:clockwiseroute} has a total length of  827 meters; while the larger loop shown in figure  \ref{fig:counterclockwiseroute} has a total length of 1,023 meters, the common areas amount to {\raise.17ex\hbox{$\scriptstyle\sim$}}514 meters, thus the vehicles in the larger loop have a chance to meet the vehicle in the shortest loop about half of the time. It is important to notice that having shared segments on the road is not a sufficient conditions for vehicles to meet and exchange data. Traffic lights, road traffic, and other urban artifact play an important role in determining wether or not two vehicles will meet. Specifically, there are 4 traffic lights around the small loop  and 6 traffic lights on the large loop. The experiments are conducted from 11am to 8pm and they factor rush- and regular hour traffic as well as pedestrian traffic at the intersections. Traffic lights and pedestrian traffic created dynamic partitioning and  voids during the experiment as it happens during the regular course of traffic in urban scenarios~\cite{rowstron2009characteristics}. While in motto, and therefore away from the roof of the parking lot, we observed a longer  wifi range  up to 318 meters.

\subsubsection{{\bf Hardware/Software Setup}} \name was installed in low-cost netbooks the \emph{Asus EeePc 1011CX} powered by an Intel Atom N80 at 1.6GHz; each node had 2GB of ram and 160GB of hard drive. Each node was retro-fitted by us with a MIMO-capable WiFi Card the \emph{Unex DNXA-92} with a specifically customized firmware to allow world-wide operations and IBSS at 5.8GHz.  The Unex DNXA-92 WiFi card is based on the Atheros  AR9280 which is supported by the Linux standard driver Ath9k. The maximum transmission power at the antenna connector is declared by the manufacturer to be  27dBm for 2.4GHz and 30dBm for the 5.8Ghz band\footnote{ During the demo only 6 nodes had the Unex DNXA-92 while the others had a standard DNXA116 thus the results factor different NICs in  hardware platform. We are planning a future test using only DNXA-92}. We used dual band omni-directional antennas the Hyperlink HG2458-7RDR-NM featuring a gain of 4.5dBi at in the 2,400-2,500MHz band and 7dBi in the 5,150-5,850MHz band, the antenna has circular polarization. All the experiments have been performed using  the 2.4GHz band (Channel 1).  Two nodes out of 10 were equipped with a second WiFi interface operating in Infrastructure mode. We used an Ubiquity Networks SR71USB which is also supported by the Linux drivers (carl9170). Furthermore two other nodes were equipped with a WiMax usb based interface connected to the UCLA-GENI WiMax testbed and operating at 2,690MHz, specifically we used the Teltonika UM62x1 which supports multiple antennas and spatial diversity. We also operate directly the WiMax base station the NEC INW-INTFC and at the time of experiments no other users were connected.  We used  an off-the-shelf Ubuntu Desktop 12.04 as operating system and \name was installed in the user space, no kernel hacks are required.  \name transmits broadcast packets in the WiFi Interfaces operating in Ad Hoc mode while tunnels the NDN traffic over IP for the other interfaces (see figure \ref{fig:packet-paths}). A \name hub is connected at other tunnel endpoint and prefers the appropriate forwarding tasks.  
The experiments were controlled by an additional 4G link provided by Clear Wireless, however such link was used only for experiment control and telemetry purposes and not a experimental link. 

\subsection{Preliminary Results}
We used rsyslog to collect the header of all the packets through the network and to log the software major events (\ie forwarding, routing, etc), this resulted in several hundred megabytes of log data helpful to gather insights and understand the capabilities of NDN. 

\begin{figure*}[htdp]
\begin{minipage}[htdp]{\textwidth}
\centering{
\subfigure[\name Info-Traffic application CDF number of Link Adaptation Layer retransmission]{
\includegraphics[width=0.47\columnwidth]{figures/Retransmission-CDF-Traffic.png}
\label{fig:trafficappcdfretransmissions}
}
\hfil
\subfigure[\name Info-Traffic application: CDF Response time  -  from the first Interest to the corresponding data ]{
\includegraphics[width=0.47\columnwidth]{figures/RTT-CDF-Traffic-LogScale.png}
\label{fig:trafficappcdfresponsetime}
}
%\hfill
%\subfigure[\name V2I: packet route]{
%\includegraphics[width=0.30\columnwidth]{figures/producer-on-the-internet}
%\label{fig:V2IRoute}
%}  
}
\caption{RTT Analysis}
\label{fig:preliminaryresults}
\end{minipage}
\end{figure*}

\subsubsection{{\bf V2V experiments }} 
Those experiments were mainly performed on November 30th and December 1st 2012, vehicles had 1 wifi interface in Ad Hoc mode. In order to support NDN using broadcast we devised mechanism for implicit acknowledgment and retransmissions that allows interest and data to make progress as detailed in section \ref{sec:wifibroadcast} the mechanism is implemented in the Link Adaptation Layer which conceptually is at layer 2.5.  \name Link Adaptation Layer manages link layer retransmissions and acknowledgments. In particular, the proposed approach tries limit the rebroadcasting of packets choosing as potential relay the nodes that are the furthest from the current one. \name LAL has embedded spatial awareness using digital maps. We designed a mechanism to allow applications to chose the degree of spatial acknowledgment; for instance at each intersection an application may require packets to be acknowledged by any or all  the road directions. The digital map and the required functionalities are implemented by the mean of a system-wide  stand-alone location service. The acknowledgment mechanism is implicit \ie the node over ears the same packet forwarded by somebody else; if no acknowledgement is detected \name link adaptation layer retransmits the packet up to \emph{max-retransmission} which was set to 7 throughout the experiments. We studied several factors:
\begin{itemize}
\item \emph{(i)} The number of retransmission needed to forward a packet by 1 hop using wifi broadcast 
\item \emph{(ii)} the response time at the application level, 
\item \emph{(iii)} the use of cache vs interest forwarding (both in regular nodes and relay-only nodes), 
\end{itemize}

Figure \ref{fig:trafficappcdfretransmissions} shows the CDF for the \name Link Adaptation Layer transmissions for the info-traffic application in different experimental scenarios (Table \ref{tab:experiments} experiments A1, A3). The chart shows that for the static case about 75\% of the packets need just one LAL retransmission. In the mobility scenario this figure goes down to about 65\% however the type of mobility (either on the P8 roof or on the roads)  has a negligible impact on the retransmissions.  It is interesting to notice that roughly 95\% of the packets are acknowledged in 5 retransmissions or less  and therefore the max-retransmission currently set to 7 is clearly an overshoot. Finally, 15\% of packets (for the static case) were acknowledged to the \name LAL before being actually transmitted and therefore they never went on the air.

The response time cumulative distribution function for the Info-Traffic application (Table \ref{tab:experiments} experiments A1, A3), is shown in figure \ref{fig:trafficappcdfresponsetime}. The chart shows that, in the static case,  about 75\% of the info-traffic interests got a response in less than 1 second. For the mobility case is interesting to note that experiments performed looping around on the roof of parking lot 8 performed worse than the experiments on the roads around campus. We believe this is due to the effect of traffic lights which introduce aggregation points and relatively long breaks in the mobility flow thus facilitating connectivity. In addition, the UCLA parking structure P8 is located in a midst of wifi access points and therefore has a very high noise background.

\begin{table}[htdp]
\caption{Cache vs Forwarding among all nodes}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
& Static & Around P8 & Around \\
& & & Campus\\
\hline
Use of Cache&2814&5280&3124\\
\hline
Interest Forward&4834&7068&17784\\
\hline
\end{tabular}
\end{center}
\label{tab:cachevsforwardinggeneral}
\end{table}%
Table \ref{tab:cachevsforwardinggeneral} shows for each mobility scenario the role of caching considering all the nodes in the network. In particular chatting contents appears to more important in mobility. This is expected as the topology changes relatively fast.  
\begin{table}[htdp]
\caption{Cache vs Forwarding among Consumers and Mules}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
& Static & Around P8 & Around \\
& & & Campus\\
\hline
Use of Cache&96&3054&1840\\
\hline
Interest Forward&715&4685&13195\\
\hline
\end{tabular}
\end{center}
\label{tab:cachevsforwardingconsumersmules}
\end{table}%
In the aim to better understand the role in-network caches for \name we  excluded from the dataset producers and analyzed the cache/forward statistics for consumer and mules. Results are shown in table  \ref{tab:cachevsforwardingconsumersmules}; the data confirms that caches are more beneficial during mobility and particularly when mobility happens in a relatively restricted area (rooftop of parking structure P8).
Observing  mule-nodes  (\ie no interests or content are sourced in this nodes) only, the role of in-network caches becomes even more prominent;  in this case about 66\% of the traffic is found in the local cached and therefore the interest is not forwarded further. 

A second reference application was tested during the experimental run, a consumer issues an interest for a picture of a certain area, the vehicle closer to that area takes a picture and delivers it back to the consumer. We implemented the application taking realtime pictures. The consumer issues an interest with a name that sounds "/picture/westwood/strathmore/" indicating it is requesting a picture from a camera that is on board of a vehicles close to the Westwood-Strathmore intersection. A vehicle in that area, if any, will turn on the camera, take a snapshot, and send it back.  While our design is far from optimal and does not employ any optimized segmentation or coding technique we were able to retrieve  51 camera shoots. Photos had an average size of 6.3KB resulting on average in 5 chunks; in order to consider a photo received all the chunks need to arrive at the consumer.  The road-photo application experienced a response time  averaging in 81 seconds for the mobile case (fig. \ref{fig:MobilityPatterns}), and 28 seconds for the static case; the median point was 55.6 seconds, and 1 second respectively. The sparse nature of our network has affected the response time for the road-photo application which suffers from disruption much more than the info-traffic application. The content for the info-traffic application is contained in one single content packet while the road-photo application requires several packets to arrive at the consumer. We believe that applying optimization techniques such as Network Coding and a more sophisticated file encoding the results can improve by far. 

\subsubsection{{\bf The role of the Infrastructure and the V2X Scenario}}  
%\note{ \bf *** WARNING *** We have very limited data on this because on the first day it failed and on the second day I forgot to turn it on, we are planning new experiments to check this. The data below is from the pre-test day Nov. 25th and November 30th}
\begin{figure}[htb]
\begin{minipage}[htb]{\columnwidth}
\centering{
\includegraphics[width=1\columnwidth]{figures/interfaceToGetPhoto.pdf}
\caption{\name V2X experiment: Link to Content allocation, each dot is a picture's chunk. }
\label{fig:V2Xlin2content}
}
\end{minipage}
\end{figure} 



%\begin{figure*}[thdp]
%\begin{minipage}[htdp]{\textwidth}
%\centering{
%\subfigure[\name V2X experiment: Mobility pattern and AP placement]{
%\includegraphics[width=0.28\columnwidth]{figures/Lot32-MultiHoming.png}
%\label{fig:car2XLot32}
%}
%\hfil
%\subfigure[\name V2X experiment: Link to Content allocation, each dot is a picture's chunk]{
%\includegraphics[width=0.35\columnwidth]{figures/interfaceToGetPhoto.pdf}
%\label{fig:V2Xlin2content}
%}
%}
%\caption{V2X Experiment}
%\label{fig:preliminaryresults}
%\end{minipage}
%\end{figure*}

In the November 25th and November 30th experiments we had few multi-homed vehicles. In particular, on November 30th two nodes were multhomed and equipped with both WiFi (V2V) and WiMax interfaces while on November 25th two nodes had  WiMax interfaces and one node had an extra WiFi interface in Infrastructure mode on top of the regular V2V interface.  The results are mainly qualitative and they are to be used mainly as a proof of concept rather than a performance evaluation. 

On November 30th 2012, 25 contents were received from the WiMax interface in one of the two multi-homed nodes and then delivered to the destination, those contents were produced by a \name node sitting on the wired network behind the WiMax ASN-Gateway.  On the november 30th experiments we were able to get 388 contents from the WiMax and 34 contents from the WiFi Infrastructure. 

In a second experiment  designed to better understand this phenomena we used two vehicles running around parking lot 32 in a clockwise fashion. On one corner of the parking structure we setup an access point and connected it to the campus infrastructure (fig. \ref{fig:car2XLot32}).  the \emph{consumer}  was equipped with 2 WiFi interfaces, one operating in  Ad-Hoc mode and a second one operating in Infrastructure mode. The \emph{producer}  was equipped with 1 WiFi interface configured in Ad Hoc mode and 1 WiMax interface. In this experiment we considered a photo fetching scenario; the consumer requests a photo to be taken by the producer at regular intervals. Interest and data packets both traveled to any interface that is available at the time of transmission. Photos were taken in realtime upon receiving the interest via the computer on-board camera, they sized between 68KB and 100KB. Each photo is split in several chunks of 1300 bytes. We accounted how on which interface chunks are transmitted as shown in figure \ref{fig:V2Xlin2content}

\subsubsection{{\bf Data survives the Producer}}  
Once a content has been spread  on the network, it survives the producer who created it - when an information goes out, its lifeline becomes independent from the lifeline of the producer. Indeed the decoupling of information and producer and the use of cache allow every nodes which got the content to use it and pass it to every consumer who will issues an interest about it, no matter when is the original producer of the data. 

As a proof of concept, we ran a session of experiments that recreated a situation where a consumer asks for a content after the only producer is gone: there is only one producer running, a consumer asks for a content and when it get it, the producer is switched off. After that, an other consumer issues the same interest, that of course ca be satisfied only by a CS of some cars around , since there is no more producer for that content.

As expected, the second consumer was able to get the desired content even if the only producer was already gone. Furthermore, thanks to the broadcast nature of the wireless communication that easily allows the spreading of a content, the satisfaction time doesn't seem to be negatively affected by the absence of the producer.




